An Empirical Study on Compressed Decentralized Stochastic Gradient Algorithms with Overparameterized Models

This paper considers decentralized optimization with application to machine learning on graphs. The growing size of neural network (NN) models has motivated prior works on decentralized stochastic gradient algorithms to incorporate communication compression. On the other hand, recent works have demonstrated the favorable convergence and generalization properties of overparameterized NNs. In this work, we present an empirical analysis on the performance of compressed decentralized stochastic gradient (DSG) algorithms with overparameterized NNs. Through simulations on an MPI network environment, we observe that the convergence rates of popular compressed DSG algorithms are robust to the size of NNs. Our findings suggest a gap between theories and practice of the compressed DSG algorithms in the existing literature.

==> figures/table_datasets.tex <==
\begin{table*}[!t]
	\centering
	\caption{
		Test-dataset Top-1 accuracies on CIFAR-10 and CIFAR-10.1 with overparameterized MLPs of varying widths. $|\mathcal{C}| \in [20, 100, 128, 200]$ co-ordinates retained. Reported test Top-1 accuracies and standard deviations averaged over 5 independent trials on $n=8$ ring topology.
	}
	\vspace{-0.2em}
	

	\resizebox{1\textwidth}{!}{%
	\centering

		\begin{tabular}{ccccc|cccc}
			\toprule
			\multirow{2}{*}{\diagbox{\# MLP Units}{\# Coordinates $\mathcal{C}$}}  & \multicolumn{4}{c|}{CIFAR-10.1}            & \multicolumn{4}{c}{CIFAR-10}  \\  \cmidrule(lr){2-9}
			       & $20$         & $100 $     & $128 $     & $200$         & $20$         & $100 $     & $128 $     & $200$     \\ \hline
			$n=2048$ &                $46.439 \pm 0.905$ & %20 coordinates %
							$47.694 \pm 0.969$ &  %100 coordinates %
							$47.282 \pm 0.657 $ &  %128 coordinates %
							$47.23 \pm 0.844$ & %200 coordinates  %
							
							$59.208 \pm 0.482$ & 
							$60.205 \pm 0.654$ & 
							$60.006 \pm 0.277$ & 
							$60.276 \pm 0.235$ \\
			
			
			
			$n=1024$ & 		$46.58 \pm 1.282$ & %
							$46.495 \pm 0.897$ & %
							$46.996 \pm 1.423$ & %
							$47.478 \pm 0.513$ & 
							
							$59.177 \pm 0.444$ & 
							$60.112 \pm 0.263$& 
							$60.131 \pm 0.598$ & 
							$59.468 \pm 0.591$ \\
			
			$n=512$ & 		$45.779 \pm 0.985$ & 
							$46.317 \pm 0.718$ & 
							$45.433 \pm 0.492$ & 
							$47.192 \pm 0.774$ & 
							
							$58.871 \pm 0.413$ & 
							$59.215 \pm 0.752$& 
							$59.329 \pm 0.635$ & 
							$58.954 \pm 0.489$ \\
									
			$n=256$ & 		$44.482 \pm 0.918$ & 
							$45.203 \pm 1.425$ & 
							$44.501 \pm 1.112$ & 
							$45.658 \pm 1.848$ & 
							
							$57.587 \pm 0.685$ & 
							$57.601 \pm 0.253$&
							$57.743 \pm 0.059$ &
						        $57.632 \pm 0.532$ \\
						        
			$n=128$ & 		$44.533 \pm 1.57$ & 
							$43.578 \pm 0.678$ & 
							$43.552 \pm 1.265$ & %
							$X $ &
							
							$55.413 \pm 0.401$ & 
							$55.679 \pm 0.592$ & 
							$55.406 \pm 0.367$ & 
							$X$ \\
			\hline 
			data~per~iteration~(MB)& $0.482$ & $2.410$ & $3.012$ & $4.820$ & $0.482$ & $2.410$ & $3.012$ & $4.820$  \\
			\bottomrule \\
		\end{tabular}%
	}
	%\caption{[Incomplete] Enter the Test dataset results on CIFAR-10.1}
	\vspace{-0.5em}
\end{table*}
